Synchronization is All You Need: Exocentric-to-Egocentric Transfer for Temporal Action Segmentation with Unlabeled Synchronized Video Pairs

We consider the problem of transferring a temporal action segmentation system initially designed for exocentric (fixed) cameras to an egocentric scenario, where wearable cameras capture video data. The conventional supervised approach requires the collection and labeling of a new set of egocentric videos to adapt the model, which is costly and time-consuming. Instead, we propose a novel methodology which performs the adaptation leveraging existing labeled exocentric videos and a new set of unlabeled, synchronized exocentric-egocentric video pairs, for which temporal action segmentation annotations do not need to be collected. We implement the proposed methodology with an approach based on knowledge distillation, which we investigate both at the feature and Temporal Action Segmentation model level. Experiments on Assembly101 and EgoExo4D demonstrate the effectiveness of the proposed method against classic unsupervised domain adaptation and temporal alignment approaches. Without bells and whistles, our best model performs on par with supervised approaches trained on labeled egocentric data, without ever seeing a single egocentric label, achieving a +15.99 improvement in the edit score (28.59 vs 12.60) on the Assembly101 dataset compared to a baseline model trained solely on exocentric data. In similar settings, our method also improves edit score by +3.32 on the challenging EgoExo4D benchmark. Code is available here: https://github.com/fpv-iplab/synchronization-is-all-you-need.

==> temp_feature_extractor.tex <==
\subsection{Effect of feature extractors}
\label{sup:ablate_feat_ext}
\begin{table}[t]
    \centering
    %\captionsetup{font=scriptsize}
    \caption{Effect of different feature extractors when the segmentation model is trained and tested on egocentric data. Domain agnostic DINOv2 features outperform EXO features (line 2 vs line 1). Performing feature distillation improves the results (line 3 vs lines 1-2) and achieves performance similar to the backbone trained on EGO features (line 3 vs line 4). Best results are reported in bold.}
    \vspace{1 mm}
    \resizebox{0.6\linewidth}{!}{
    \begin{tabular}{cccrrrrr}
    %\hline
    \textbf{Backbone} & \textbf{Train} & \textbf{Feature Dist.} & \textbf{Edit} & $\bf{F1_{10}}$ & $\bf{F1_{25}}$ & $\bf{F1_{50}}$ & \textbf{MoF} \\
    \hline
    TSM                                   & EXO                                &                                                        & 22.83                     & 20.57                     & 17.05                     & 10.92                     & 24.56                     \\
DINOv2                                   &  /                           &                               &  26.42 &26.50&22.16&18.84&33.47\\
TSM           &                      EXO                                 & \checkmark                       & 28.61 & 30.60 & \textbf{26.39} & \textbf{18.87}& 36.06 \\

TSM             &             EGO         &                               & \textbf{29.25}                     & \textbf{31.06}                     & 25.40                     & 17.47                     & \textbf{36.60}                     \\
\hline
\end{tabular}}
\label{tab:feat_ext_results}


\end{table}
\Cref{tab:feat_ext_results} reports the results of experiments aimed at assessing the effect of different feature extractors. For fair comparisons, for all approaches, temporal action segmentation models have been trained and tested using egocentric data, regardless of the data used to train the corresponding feature extractor, leading to a set of egocentric oracles, which differ only on the feature extractors. 
Methods obtained by training a TSM model on supervised exocentric data only achieve the worst performance %(e.g., line 1 obtains an edit score of $22.83$).
(e.g. edit score of $22.83$)
Models based on the domain-agnostic DINOv2 feature extractor obtain better results %(edit score of $26.42$ vs $22.83$ and an MoF of $33.47$ vs $24.56$ when comparing line 2 to line 1). 
(edit score of $26.42$ vs $22.83$, MoF of $33.47$ vs $24.56$). 
The best overall results are obtained by an ego-oracle training the TSM module directly on egocentric features %(line 4 obtained an edit score of $29.25$). 
(edit score of $29.25$). 
%
Interestingly, distilling the exocentric model with unlabeled synchronized exo-ego data allows to achieve similar performance %(line 4 has an edit score of $28.61$ and even outperforms the ego-oracle - line 3 - w.r.t. $F1_{25}$ and $F1_{50}$ measures)
(edit score of $28.61$ and even outperforms the ego-oracle $F1_{25}$ and $F1_{50}$ measures), which highlights the ability of the feature distillation process to partially fill the representation gap. 
See Sections~\ref{supp:ablate_exo_ego_data} of supp. for additional experiments on training data.
